A Hybrid Approximation to the Marginal Likelihood

Computing the marginal likelihood or evidence is one of the core challenges in Bayesian analysis. While there are many established methods for estimating this quantity, they predominantly rely on using a large number of posterior samples obtained from a Markov Chain Monte Carlo (MCMC) algorithm. As the dimension of the parameter space increases, however, many of these methods become prohibitively slow and potentially inaccurate. In this paper, we propose a novel method in which we use the MCMC samples to learn a high probability partition of the parameter space and then form a deterministic approximation over each of these partition sets. This two-step procedure, which constitutes both a probabilistic and a deterministic component, is termed a Hybrid approximation to the marginal likelihood. We demonstrate its versatility in a plethora of examples with varying dimension and sample size, and we also highlight the Hybrid approximation's effectiveness in situations where there is either a limited number or only approximate MCMC samples available.

==> algo.tex <==

% draw samples from the posterior distribution, evaluate \Psi(u) for each of these

% fit the pairs into a decision tree

% extract the partition from the tree
% use the constant approximation described in previous section to obtain 
% the approximation of the integral = marginal likelihood

\subsection{Algorithm Description}
Until this point, the representative point within each partition has simply been the fitted value for each partition returned from the CART model. When $\{(u_j , \Psi(u_j))\}_{j=1}^J$ is fed into the tree, it attempts to optimize the sum of squared errors as in Eq.\,\eqref{eq:SSE}. Note, however, that our eventual objective is to best approximate the functional $\log \int_A e^{-\Psi}$, and it is not unreasonable to suspect that the optimal value for $A_k$ chosen by the regression tree model may not be a suitable choice for our end goal, especially for higher dimensions. Simulations in higher dimensions indeed confirm this. Before suggesting a remedy, we offer some additional understanding into the approximation mechanism that guides us toward an improved choice. To that end, write $\wt{F}_A$ from Eq.\,\eqref{eq:Fhat} as  
\begin{align*}
    \widehat{F}_A = \log \bigg[\sum_{k=1}^K e^{-c_k^\star} \, p_k \bigg] + \log \mu(A) 
    :\, = \widehat{G} + \log \mu(A),
\end{align*}
where recall $\mu(B) = \mbox{vol}(B)$ is the Lebesgue measure of a Borel set $B$, and we define $p_k :\,= \mu(A_k)/\mu(A)$. We can also write $F_A = G + \log \mu(A)$, with 
\begin{align*}
    G &:\,= \log \bigg[ \frac{1}{\mu(A)} \int_A e^{- \Psi(u) } du \bigg] \\
    &= \log \bigg[\sum_{k=1}^K p_k \frac{1}{\mu(A_k)} \int_{A_k} e^{- \Psi(u) } du \bigg] \\
    &= \log \bigg[ \sum_{k=1}^K e^{-c_k} \, p_k \bigg],
\end{align*}
where 
\be 
e^{-c_k} = \frac{1}{\mu(A_k)} \int_{A_k} e^{- \Psi(u) } du = \bbE_{U_k \sim \mbox{Unif}(A_k)} \big[e^{-\Psi(U_k)} \big].
\ee
Thus, for $\wt{G}$ to approximate $G$, we would ideally like to have each $c_k^\star$ chosen so that $e^{-c_k^\star}$ targets $e^{-c_k}$. Importantly, the above exercise suggests the appropriate scale to perform the approximation -- rather than working in the linear scale as in Eq.\,\eqref{eq:SSE}, it is potentially advantageous to work in the exponential scale. 


%As a result, for a partition set $A_k$, the optimal value $c_k^\star$ is chosen on the same scale as $\Psi(\cdot)$. However, the integrand that we approximate in (\ref{eq:Z}), $e^{-\Psi(u)}$, is on an exponential scale. Therefore,  

% Another aspect of the initial algorithm that we now consider in more depth is the partitioning scheme. Currently, the set of MCMC samples that we use to fit the CART model provide a partition over the parameter space. We then compute a local approximation $\Psi$ over each of the partition sets as an intermediate step for computing they hybrid estimator. This two-step process of carving up the underlying space using a tree and computing local approximations over each of the terminal nodes has been used in other problem settings as well. In \cite{ma_2017}, Ma approaches the problem of modeling conditional densities by proposing a two-stage procedure of first partitioning the predictor space using an Optional Polya Tree \cite{wong_ma_2010}, and then locally generating the conditional distribution by a multi-scale nonparametric density model on each of the partition sets learned from the first step. 

% With the CART model returning a partition of the parameter space, we see that this yields a computationally efficient approximation to the marginal likelihood. However, in order to further exploit this process, we look to areas of the parameter space that have already been identified as regions of posterior probability and explore these areas more fully by repeatedly partitioning these regions. With this finer partition in place, each set with its own systematically chosen representative point, the integral computed over each of these partition sets will ideally give an improved estimate of the marginal likelihood. 


\subsubsection{Choosing the Representative Point}

Based on the above discussion, we define a family of objective functions
\begin{align}\label{eq:obj_Q}
    Q_k(c) = \sum_{u \in A_k} \frac{|e^{-\Psi(u)} - e^{-c}|}{e^{-\Psi(u)}}, \quad c \in A_k,
\end{align}
one for each partition set $A_k$ returned by the tree, and set $c_k^\star = \mathrm{argmin}_{c} Q_k(c)$. We experimented with a number of different metrics before zeroing in on the above relative error criterion in the exponential scale. Minimizing \eqref{eq:obj_Q} is a weighted $\ell_1$ problem and admits a closed-form solution. 

Thus, our overall algorithm can be summarized as follows. We obtain samples $u_1, \ldots, u_J$ from $\gamma$, and feed $\{(u_j, \Psi(u_j)\}_{j=1}^J$ through a tree to partition the bounding box $A$ of the samples. Then, rather than using the default fitted values returned by the tree, we take the representative value $c_k^\star$ within each $A_k$ as the minimizer of $Q_k$. These $c_k^\star$s are then used to compute $\wt{F}_A$ as in \eqref{eq:Fhat} -- note that $\wt{F}_A$ can be stably computed using the log-sum-exp trick. Finally, we declare $\wt{F}_A$ as $\log \wt{\m Z}$, our estimator of $\log \m Z$. 
%In practice, $c$ is chosen from a grid of candidate points from $A_k$ which can then be evaluated using the objective function $Q(\cdot, k)$. 

%In addition, it is computationally beneficial to consider these quantities in the log scale, as the exponential terms in both the Hybrid approximation and the objective function result in numerical instability. The form of the estimator conveniently allows us to use the log-sum-exp trick to stabilize this calculation,
%\begin{align*}
%	& \log \wt{\m Z} = \log \left[ \sum_{k=1}^K \int_{A_k} e^{-c_k^\star} \, du \right].
%\end{align*}


\iffalse
\subsubsection{Repartitioning scheme}
After modifying the initially discussed algorithm by adopting the objective function in (\ref{eq:obj_Q}) to choose each partition set's representative point, we obtain the approximation, $\wt{\Psi}_1(u) = \sum_{k=1}^K c_k^{\star} \ 1_{A_k}(u)$, which we refer to as the \textit{stage-1 approximation}. Note that this is symbolically identical to the approximation given in (\ref{eqn:constant_approx}) but with a different choice of $c_k^\star$. Like before, let $\m A = \{ A_1, A_2, \ldots, A_K \}$ be the partition set learned from the CART model, where each partition $A_k$ contains $N_k$ points. For a given point $u \in \m U$, we can decompose $\Psi(u)$ as follows, 
\begin{align*} 
    \Psi(u) = \wt{\Psi}_1(u) + \varepsilon(u).
\end{align*}
Here, $\varepsilon$ is the residual term. Rearranging, we have the following expression for the residual,  
\begin{align} \label{eq:residual}
    \varepsilon(u) = \Psi(u) - \sum_{k=1}^K c_k^{\star} \ 1_{A_k}(u).
\end{align}
For the next step of the algorithm, we look to iteratively fit the residual using a similar approximation scheme to the one presented in the previous algorithm. In particular, instead of solely approximating $\Psi(u)$ on each of these partitions, we also fit the residual term in hopes of recovering a better approximation to $\Psi$. Consider the partition $A_k$, from which we sample $N_k' = M \cdot N_k$ points uniformly from $A_k$ (for a fixed $M$) and use (\ref{eq:residual}) to compute the residual. Forming the following pairs, $\{ (u_{r}^{(k)}, \varepsilon(u_{r}^{(k)})) \}$, $r = 1, \ldots, N_k'$, we can once again fit a CART model which admits a partition $\m A_k = \{ A_{k1}, A_{k2}, \ldots, A_{k s_k}\}$, such that $\bigcup_{j=1}^{s_k} A_{kj} = A_k$. Like before, we give a locally constant approximation to $\varepsilon$ over each of the sub-partition sets of $A_k$ returned from the regression tree.
\begin{align} \label{eq:resid_local_approx}
    \varepsilon(u) \approx \hat{\varepsilon}(u) = \sum_{j=1}^{s_k} e_{kj}^\star \ 1_{A_{kj}} (u),
\end{align}
where $e_{kj}^\star$ is chosen to be a representative point of $A_{kj}$. Repeating this process for each of the $K$ partitions, we can then write the \textit{stage-2 approximation} to $\Psi$ as
\begin{align} \label{eq:stage2_approx}
    \wt{\Psi}_2(u) &= \wt{\Psi}_1(u) + \hat{\varepsilon} \\
    &= \sum_{k=1}^K c_k^\star \ 1_{A_k}(u) + \sum_{k=1}^K \sum_{j=1}^{s_k} e_{kj}^{\star} \ 1_{A_{kj}}(u).
\end{align}
Taking $c_{kj}^\star = c_k^{\star} + e_{kj}^{\star}$, we can write this approximation so that it resembles stage-1 approximation, 
\begin{align} \label{eq:stage2_approx_equiv}
    \wt{\Psi}_2(u) = \sum_{k=1}^{K} \sum_{j=1}^{s_k} c_{kj}^{\star} \ A_{kj}(u).
\end{align}
Noting that the expression in (\ref{eq:stage2_approx_equiv}) is essentially the original approximation in (\ref{eqn:constant_approx}), we can directly apply the results derived in (\ref{eqn:constant_approx_partition}) and (\ref{eqn:ml_approx}) to obtain an updated approximation to the marginal likelihood, 
\begin{align} \label{eq:stage2_ml_approx}
    \wt{\m Z} = \int e^{-\wt{\Psi}_2(u)} du = \sum_{k=1}^{K} \sum_{j=1}^{s_k} \int_{A_{kj}} e^{-c_{kj}^\star} \ du,
\end{align}
where the integral can be analytically evaluated over the $d$-dimensional hypercube that defines $A_{kj}$. Taking $\wt{\m Z}$ as an approximation for $\m Z$, we then have an updated approximation that has taken into account the residual of $\Psi$ over each of the sub-partition sets. With this recursive architecture in place, we can carry out this repartitioning scheme again by defining $\varepsilon = \Psi - \wt{\Psi}_2$ and following the process of sampling uniformly from each of the sub-partitions obtained from the previous stage. Then, the \textit{stage-3 approximation} can be written as
\begin{align} \label{eq:stage3}
    & \wt{\Psi}_3(u) = \sum_{k = 1}^{K} \sum_{j = 1}^{s_k} \sum_{l = 1}^{n_{kj}} c^{\star}_{kjl} \ 1_{A_{kjl}}(u),
\end{align}
where $c_{kjl}^\star = c^{\star}_k + e^{\star}_{kj} + f^{\star}_{kjl}$. It is easy to see that this process can be continued indefinitely, where each successive stage results in finer and finer partitions of the parameter space. However, this recursive partitioning process becomes prohibitively expensive beyond a few iterations. Empirically, we have found that in most cases, forming the stage-3 approximation, i.e, re-partitioning an additional two times after fitting the initial CART model, yields a partition that provides enough depth within high probability regions and carves up the parameter space sufficiently. 

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\textwidth]{figs/sec_stage.png}
  \caption{Visual representation of partitioning procedure with the MCMC samples plotted. Left: partition space after initial partitioning. Right: repartitioning each of the partitions obtained in the previous step. The partitions obtained during the second stage are shown in blue.}
  \label{fig:second_stage}
\end{figure}
\fi

\iffalse %%% remove any mention of repartitioning for now for this iteration of the algorithm (double check?)
In addition, it is computationally beneficial to consider these quantities in the log scale, as the log-likelihood term in the approximation quickly results in stability issues. The form of the estimator at each stage conveniently allows us to use the log-sum-exp trick to perform a stable calculation of the hybrid estimator. To be exact, the \textit{stage-3 approximation} in (\ref{eq:stage3}) can be used to construct the hybrid estimator in the log scale as follows,
\begin{align*}
    & \log \wt{\m Z} = \log \left[ \sum_{k=1}^K \sum_{j=1}^{s_k} \sum_{l=1}^{n_{kj}} \int_{A_{kjl}} c^{\star}_{kjl} \ du \right].
\end{align*}
In practice, we can simplify the final approximation by defining the hybrid estimator by taking the mean of the estimators over each of the stages, 
\begin{align} \label{eq:hybrid_final}
     \log \m Z^\star = \frac{1}{3} \sum_{i = 1}^3 \log \wt{\m Z}_i,
\end{align}
where $\wt{\m Z}_i$ is the approximation for the marginal likelihood that uses the \textit{stage-$i$ approximation}, $\wt{\Psi}_i$, to approximate $\Psi$. 
\fi


\iffalse
\subsubsection{Choosing the Representative Point}

Previously, when approximating the negative log posterior $\Psi$, we use the objective function $Q(c, k)$ to find a partition set's representative point. During this repartitioning process, however, we pivot to fitting the residuals, so we define a slightly modified version of the objective function to select representative points.

For simplicity, consider the case for which we are trying to compute the stage-2 approximation, and we already have a sub-partition $\m A_k = \{ A_{k1}, A_{k2}, \ldots, A_{k s_k}\}$ in place for the partition set $A_k$. In order to compute the approximation to the residual in (\ref{eq:resid_local_approx}), we require that for each sub-partition set $A_{kj}$ of $A_k$, $e_{kj}^\star$ is some representative point of the partition. We define the following objective function,
\begin{align*}
    R(c, k) = \sum_{u \in A_k} \frac{|e^{-\varepsilon(u)} - e^{-c}|}{e^{-c}}.
\end{align*}
Then, we choose $e_{kj}^\star = \mathrm{argmin}_{c} \  R(c, kj)$. In practice, $c$ is chosen from a grid of candidate points from $A_{kj}$ which can then be evaluated using the objective function $R(\cdot, k)$. 

\pagebreak
\fi



    \begin{algorithm}
    \caption{Hybrid Approximation}\label{alg:hybrid}
    \hspace*{\algorithmicindent} \textbf{Input:} Sampler for $\gamma$, method for evaluating $\Psi$ \\
    \hspace*{\algorithmicindent} \textbf{Output:} Estimate of the log marginal likelihood
    \begin{algorithmic}[1]
    \State Sample  $\{u_j\}_{j=1}^J$ from $\gamma$
    \State Fit $\{ (u_j, \Psi(u_j)) \}_{j=1}^J$ using a regression tree
    \State From the fitted tree, extract the dyadic partition $\mathcal{A} = \{ A_1, A_2, \ldots, A_K\}$ of the bounding box $A = \otimes_l \left[ \min \{ u^{(l)}_{j} \}, \max \{ u^{(l)}_{j} \} \right]$ determined by the samples, with $A_k = \prod_{l=1}^d [a_k^{(l)}, b_k^{(l)}]$
    \For{$k \in \{ 1 , \ldots,  K \}$}
        \State $c_k^\star \gets \mathrm{argmin}_{c \in A_k} \log Q_k(c)$
        \State $\wt{\mathcal{Z}}_k \gets e^{-c_k^\star} \ \prod_{l=1}^d \big(b_k^{(l)} - a_k^{(l)}\big)$
    \EndFor
    \State Use the log-sum-exp trick to compute the final estimator, $\log \wt{\mathcal{Z}} = \texttt{log-sum-exp} \left( \log \hat{\mathcal{Z}}_1, \ldots, \log \hat{\mathcal{Z}}_K  \right)$
    \end{algorithmic}
    \end{algorithm}



%%%% algorithm visual
\iffalse
\begin{algorithm}[h!]
\DontPrintSemicolon
\SetAlgoLined
\SetNoFillComment
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{Samples $\{u_j\}_{j=1}^J$ from $\gamma$, method for evaluating $\Psi$ }
\Output{Estimate $\log \wt{\m Z}$ of the log marginal likelihood}
\BlankLine
\setstretch{1.0}
    Fit $\{ (u_j, \Psi(u_j)) \}_{j=1}^J$ using a regression tree\;
    %Define the compactification of $\m U$ as $A$, where $A = \otimes_d \left[ \min \{ u_{d(j)} \}, \max \{ u_{d(j)} \} \right]$, $1 \leq j \leq J$\;
    From the fitted tree, extract the dyadic partition $\m A = \{ A_1, A_2, \ldots, A_K\}$ of the bounding box $A = \otimes_d \left[ \min \{ u_{d(j)} \}, \max \{ u_{d(j)} \} \right]$ determined by the samples, with $A_k = \prod_{j=1}^d [a_k^{(d)}, b_k^{(d)}]$\;
    \For{$k \gets 1 \ \mathbf{to} \ K$}{
        $c_k^\star \gets \mathrm{argmin}_{c \in A_k} \log Q_k(c)$\;
        \setstretch{1.7}
        $\wt{\m Z}_k \gets e^{-c_k^\star} \ \prod_{j=1}^d \big(b_j^{(d)} - a_j^{(d)}\big)$\;
    }
    % $\log \wt{\m Z} \gets \log \sum_k \wt{\m Z}_k$\;
    Use the log-sum-exp trick to compute the final estimator, $\log \wt{\m Z}$, $\log \wt{\m Z} = \texttt{log-sum-exp} \left( \log \hat{\m Z}_1, \ldots, \log \hat{\m Z}_K  \right)$\;
\caption{Hybrid Approximation}
\end{algorithm}
\fi





%%%% algorithm figure ------------------------------------------------------------

\iffalse
\begin{algorithm}[H] \label{alg1}
\DontPrintSemicolon
\SetAlgoLined
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{Number of posterior samples $J$, sampler for $\gamma(u)$, expression for $\Psi(u)$}
\Output{Approximate Marginal Likelihood, $\wt{\m Z}$}
\BlankLine
\setstretch{1.1}
    \textrm{Sample} $u_1, u_2, \ldots, u_J \sim \gamma(u)$\;
    \textrm{Fit} $\{ (u_1, \Psi(u_1)), (u_2, \Psi(u_2)), \ldots, (u_J, \Psi(u_J))\}$  using a regression tree\;
    \textrm{Extract} partition $\{ A_1, A_2, \ldots, A_K\}$ from fitted tree\;
    \For{$k \gets 1 \ \mathbf{to} \ K$}{
        $c_k^\star \gets \mathrm{argmin}_{c_k} \log Q(c_k)$\;
        $\wt{\m Z}_k \gets e^{-c_k^\star} \cdot \mu(A_k)$\; 
    }
    $\wt{\m Z} \gets \wt{\m Z}_1 + \cdots + \wt{\m Z}_K$
\caption{Tree-Based Approximation}
\end{algorithm}
\fi




%%%% constant approximation numerical results ------------------------------------------------------------

==> twodim.tex <==


\subsection{Partitioning in Two Dimensions} \label{sec:two_dim}

Before moving into higher dimensions, we provide an illustration of the process described in the previous section in 2 dimensions, where the partitioning can be easily visualized. Suppose $\gamma$ is a density on $\mathbb{R}^2$ supported on $\m U \subseteq \mathbb{R}^2$, and $u_j \sim \gamma$ for $j = 1, \ldots, J$. Forming the pairs, $\{(u_j, \Psi(u_j))\}_{j=1}^J$, we then fit a CART model to these points and extract the decision rules, which form a dyadic partition of the aforementioned bounding box $A \subseteq \m U$. Denote the partition as $\m A = \{ A_1, \ldots, A_K \}$. Plotting the sampled points and overlaying the partitions learned from the regression tree, we observe in Figure \ref{fig:twod_partition} that areas of $\m U$ with a high concentration of points coincide with regions that are more finely partitioned by the regression tree. Taking $\gamma$ to be a posterior distribution, we see that this behavior of partitioning areas of greater posterior mass is desirable in producing a better approximation. Equipped with the partition $\m A$, we need only to determine the representative point of each partition set in order to form the approximation to $\Psi$.

Recall that CART fits a constant for each point within a given partition set. At any given stage, the CART model will search for the optimal predictor value, $u = (u_1, u_2)$, on which to partition the remaining points such that the sum of squares error (SSE) between the response, $\Psi(u)$, and the predicted constant is minimized. In particular, to partition data into two regions $A_1$ and $A_2$, the objective function is given as 
\begin{align} \label{eq:SSE}
    & SSE = \sum_{u_i \in A_1} (\Psi(u_i) - c_1)^2 + \sum_{u_i \in A_2} (\Psi(u_i) - c_2)^2.
\end{align}
Upon minimization of the SSE, the resulting partition sets $A_1$ and $A_2$ have fitted values $c_1$ and $c_2$, respectively. For each partition set $A_k \in \m A$, a natural choice for the representative point $c_k^\star$ is the fitted value for $A_k$ produced by the tree-fitting algorithm. Following this two-step process of using CART to obtain both the partition and the fitted values for each of the partition sets and then plugging these into Eq. (\ref{eqn:ml_approx}), we obtain the Hybrid approximation to the marginal likelihood.

\subsubsection{Conjugate Normal Model} \label{sec:conjugate2d}

We consider the following conjugate normal model: $y_{1:n} \mid \mu, \sigma^2 \sim \m N(\mu, \sigma^2)$, $\mu \mid \sigma^2 \sim \m N(m_0, \sigma^2 / w_0)$, $\sigma^2 \sim \m{IG}(r_0 / 2, s_0 / 2)$, where $\m{IG}(\cdot, \cdot)$ denotes the inverse-gamma distribution. In order to compute the Hybrid estimator, we require samples from the posterior distribution and a way to evaluate $\Psi$. In this example, the posterior distribution of $u = (\mu,\sigma^2)$ is known, and since the likelihood and prior are specified, the evaluation of $\Psi$ is straightforward. With this architecture in place, we feed the pairs, $\{ (u_{j}), \Psi(u_{j}) \}_{j=1}^J$, through CART to obtain a partition over the parameter space and each partition set's representative point. Then, we use Eq. (\ref{eqn:ml_approx}) to compute the final approximation.
\begin{table}[h]
\caption{\textit{Normal Inverse-Gamma Example. We report the mean, standard deviation, average error (AE, truth - estimated), and the root mean squared error (RMSE), taken over 100 replications. Each replication has 50 observations and 1000 posterior samples. The true log marginal likelihood is -113.143. Estimators include the Harmonic Mean estimator (HME), Corrected Arithmetic Mean estimator (CAME), Bridge Sampling estimator (BSE), and the Hybrid estimator (HybE).}}
\label{tab:nig2d}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\textbf{Method}  & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} & \multicolumn{1}{l|}{\textbf{AE}} & \multicolumn{1}{l}{\textbf{RMSE}} \\ \hline
log HME          & -104.762                    & 0.733                    & -8.381                    & 8.431      \\
log CAME         & -112.704                    & 0.048                    & -0.439                    & 0.441      \\
log BSE          & -113.143                    & 0.006                    & 0                         & 0.006      \\
log HybE         & -113.029                    & 0.025                    & -0.114                    & 0.117                            
\end{tabular}%
}
\end{center}
\end{table}

Table \ref{tab:nig2d} shows results for the Hybrid estimator and a number of other competing methods. Here, the true log marginal likelihood can be computed in closed form, so we have direct comparisons to the ground truth. All estimators except for the Harmonic Mean estimator give accurate approximations to the log marginal likelihood. 


%\subsubsection{Tree Approximation} \label{sec:og_mvn}
%Naturally, we want to check the accuracy of the Hybrid estimator as the dimension of the parameter space grows. We consider the standard linear regression model $y = X\beta + \varepsilon$, where $X \in \mathbb{R}^{n\times d}$, $\beta \in \mathbb{R}^d$, and $\varepsilon \sim \m N(0, \sigma^2 I_n)$. We place a multivariate normal prior on the parameter of interest, $\beta \mid \sigma^2, \lambda \sim \m N_d( 0, \sigma^2 \lambda^{-1} I_d)$. For $d = 10$, however, the Hybrid estimator already begins to suffer, calling for more methodical consideration of the initially proposed algorithm. We focus now on the approximation to $\Psi$ that the regression tree produces for each partition. 

% begin theory.tex content -----------------------------------------------------










\iffalse
Table \ref{tab:mvn-basic} shows the results for $d = 10$. As before, the CAME and the BSE both produce reliable estimates. In contrast, the accuracy of the hybrid estimator suffers quite drastically, indicating that the initially proposed algorithm would benefit from some more methodical consideration.
\begin{table}[h]
\caption{\textit{Mean and standard deviation of the estimates for the 10-dimensional multivariate normal example, taken over 100 replications. Each replication has 100 observations and 1000 posterior samples. The true log marginal likelihood is -257.7619. We report the average error (AE), truth - estimate, and the root mean squared error (RMSE).}}
\label{tab:mvn-basic}
\begin{center}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|c|c|c|c}
\textbf{Method}   & \multicolumn{1}{l|}{\textbf{Mean}} & \multicolumn{1}{l|}{\textbf{SD}} & \multicolumn{1}{l|}{\textbf{AE}} & \multicolumn{1}{l}{\textbf{RMSE}} \\ \hline
log HME           & -219.326                      & 1.084                        & -38.436                       & 38.451                     \\
\textbf{log CAME} & \textbf{-257.762}             & \textbf{0.003}               & \textbf{0}                    & \textbf{0.003}             \\
log BSE           & -257.761                      & 0.011                        & -0.001                        & 0.011                       \\
log HybE          & -254.404                      & 0.224                        & -3.358                        & 3.366                            
\end{tabular}%
}
\end{center}
\end{table}
\fi





